A Theoretical Framework for Graph-based Digital Twins for Supply Chain Management and Optimization

Supply chain management is growing increasingly complex due to globalization, evolving market demands, and sustainability pressures, yet traditional systems struggle with fragmented data and limited analytical capabilities. Graph-based modeling offers a powerful way to capture the intricate relationships within supply chains, while Digital Twins (DTs) enable real-time monitoring and dynamic simulations. However, current implementations often face challenges related to scalability, data integration, and the lack of sustainability-focused metrics. To address these gaps, we propose a Graph-Based Digital Twin Framework for Supply Chain Optimization, which combines graph modeling with DT architecture to create a dynamic, real-time representation of supply networks. Our framework integrates a Data Integration Layer to harmonize disparate sources, a Graph Construction Module to model complex dependencies, and a Simulation and Analysis Engine for scalable optimization. Importantly, we embed sustainability metrics - such as carbon footprints and resource utilization - into operational dashboards to drive eco-efficiency. By leveraging the synergy between graph-based modeling and DTs, our approach enhances scalability, improves decision-making, and enables organizations to proactively manage disruptions, cut costs, and transition toward greener, more resilient supply chains.

==> designs.tex <==
\begin{AIbox}{Main theoretical result}
When the induced distribution of rewards under the pre-trained $\pibase$ is anti-concentrated, and $\pibase$ is heterogeneous: \textbf{(i)} for a fixed test-time compute budget $H$, verifier-based RL and search algorithms outperform \textbf{\emph{any}} verifier-free algorithm; \textbf{(ii)} the gap between the two grows as $\sqrt{H}$ as we scale both data $n = \Omega(H)$, and test compute $H$.
\end{AIbox}

\begin{tcolorbox}[colback=green!5!white,colframe=black,boxsep=0pt,top=4pt,bottom=4pt,left=3pt,right=3pt]
\begin{property}[Bi-level rewards]
\label{prp:bi-level-reward} For any trajectory $\tau$, rewards are binary and non-decreasing, \textit{i.e.} $\forall h \in [H]$, $r_{h+1} (\bs_{h+1}, a_{h+1}) \geq r_{h} (\bs_h, a_h)$, (example in Figure~\ref{fig:bi-level-reward-example}). 
\end{property}
\end{tcolorbox}
